JMMMU: A Japanese Massive Multi-discipline Multimodal Understanding Benchmark for Culture-aware Evaluation

Accelerating research on Large Multimodal Models (LMMs) in non-English languages is crucial for enhancing user experiences across broader populations. In this paper, we introduce JMMMU (Japanese MMMU), the first large-scale Japanese benchmark designed to evaluate LMMs on expert-level tasks based on the Japanese cultural context. To facilitate comprehensive culture-aware evaluation, JMMMU features two complementary subsets: (i) culture-agnostic (CA) subset, where the culture-independent subjects (e.g., Math) are selected and translated into Japanese, enabling one-to-one comparison with its English counterpart MMMU; and (ii) culture-specific (CS) subset, comprising newly crafted subjects that reflect Japanese cultural context. Using the CA subset, we observe performance drop in many LMMs when evaluated in Japanese, which is purely attributable to language variation. Using the CS subset, we reveal their inadequate Japanese cultural understanding. Further, by combining both subsets, we identify that some LMMs perform well on the CA subset but not on the CS subset, exposing a shallow understanding of the Japanese language that lacks depth in cultural understanding. We hope this work will not only help advance LMM performance in Japanese but also serve as a guideline to create high-standard, culturally diverse benchmarks for multilingual LMM development. The project page is https://mmmu-japanese-benchmark.github.io/JMMMU/.

==> Styles/sections/src/_analysis_cs_english.tex <==
% \begin{table*}[t]
% \centering
% \footnotesize
% \centering
%      {\tabcolsep = 0.5mm
%     \begin{tabular}{@{}lrrrrrrrrrr@{}} \toprule
% Model & CS (EN) & CS (JA) & Art (EN) & Art (JA) & Heri (EN) & Heri (JA) & Jpn Hist (EN) & Jpn Hist (JA) & WRD Hist (EN) & WRD Hist (JA) \\
% \midrule
% CogVLM2-19B & 51.3 & 39.7 & 44.0 & 39.3 & 50.7 & 24.0 & 40.0 & 36.0 & 70.7 & 59.3 \\
% EvoVLM JP v2 & 41.8 & 45.2 & 38.0 & 44.0 & 34.7 & 40.0 & 38.7 & 42.0 & 56.0 & 54.7 \\
% idefics2-8b & 50.7 & 37.0 & 42.7 & 40.7 & 48.0 & 24.0 & 42.7 & 30.0 & 69.3 & 53.3 \\
% idefics3-8b & 46.7 & 42.8 & 47.3 & 43.3 & 34.7 & 24.7 & 36.0 & 42.0 & 68.7 & 61.3 \\
% InternVL2-2B & 37.3 & 29.2 & 38.0 & 31.3 & 28.0 & 22.7 & 28.7 & 30.7 & 54.7 & 32.0 \\
% InternVL2-8B & 47.2 & 42.5 & 42.7 & 41.3 & 42.7 & 38.0 & 36.0 & 35.3 & 67.3 & 55.3 \\
% LLaVA-OV-0.5B & 31.7 & 23.3 & 29.3 & 22.7 & 22.0 & 22.7 & 35.3 & 24.0 & 40.0 & 24.0 \\
% LLaVA-OV-7B & 46.2 & 43.0 & 41.3 & 36.0 & 38.7 & 30.7 & 36.0 & 37.3 & 68.7 & 68.0 \\
% LLaVA-1.6-13B & 46.5 & 33.7 & 34.7 & 32.0 & 47.3 & 24.0 & 37.3 & 32.0 & 66.7 & 46.7 \\
% LLaVA-1.6-34B & 52.2 & 43.2 & 46.0 & 42.0 & 46.7 & 36.0 & 43.3 & 40.7 & 72.7 & 54.0 \\
% Mantis 8B & 46.7 & 39.5 & 45.3 & 42.0 & 37.3 & 30.0 & 39.3 & 35.3 & 64.7 & 50.7 \\
% Phi-3.5v & 43.0 & 34.3 & 40.0 & 37.3 & 35.3 & 27.3 & 34.7 & 35.3 & 62.0 & 37.3 \\
% Phi-3v & 41.0 & 26.5 & 39.3 & 31.3 & 33.3 & 18.7 & 30.7 & 29.3 & 60.7 & 26.7 \\
% xGen-MM & 48.8 & 28.2 & 45.3 & 30.0 & 38.0 & 20.7 & 39.3 & 22.7 & 72.7 & 39.3 \\
% LLaVA-Calm2 & 37.8 & 41.5 & 41.3 & 42.7 & 30.0 & 36.7 & 29.3 & 40.0 & 50.7 & 46.7 \\
% Gemini1.5Pro & 59.0 & 60.3 & 56.0 & 54.7 & 54.7 & 55.3 & 48.7 & 55.3 & 76.7 & 76.0 \\
% GPT-4o & 73.5 & 66.7 & 66.7 & 60.7 & 75.3 & 70.7 & 62.0 & 58.7 & 90.0 & 76.7 \\
% \bottomrule
% \end{tabular}
% \caption{\small{\textbf{Check for Japanese culture english !!!!}}}}
% \label{table:single_IN}
% \end{table*}


==> Styles/sections/src/before_and_after_translation.tex <==
% \begin{figure}[tb]
%     \centering
%     \includegraphics[width=0.99\linewidth]{Styles/sections/figures/before_and_after_translation.pdf}
%     \vspace{-5mm}
%     \caption{
%         \textbf{The response difference between English and Japanese.}
%         In Japanese, GPT-4o goes against the instruction that asks to answer directly and generates its reasoning process, leading to a correct answer.
%         \so{いい感じの見せ方が思い付いてないので後ほど変更します}
%     }
%     \label{fig:before_and_after_translation}
% \end{figure}


==> Styles/sections/src/error.tex <==


\begin{figure}[t]
    \centering
    \includegraphics[width=0.99\linewidth]{Styles/sections/figures/error.png}
    \vspace{-3mm}
    \caption{
        \textbf{Error in translation \so{tmp}}
    }
    \label{fig:error}
\end{figure}


==> Styles/sections/src/heron.tex <==

\begin{figure}[H]
    \centering
    \includegraphics[width=0.99\linewidth]{Styles/sections/figures/heron_jmmmu.png}
    \vspace{-3mm}
    \caption{
        \textbf{Heron Bench and JMMMU}
    }
    \label{fig:heron}
    % \vspace{-1em}
\end{figure}


==> Styles/sections/src/lack_of_knowledge.tex <==
% \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.99\linewidth]{Styles/sections/figures/lack_of_knowledge.pdf}
%     \vspace{-3mm}
%     \caption{
%         \textbf{Example of Lack of Knowledge.}
%     }
%     \label{fig:lack_of_knowledge}
% \end{figure}





==> Styles/sections/src/perceptual_error.tex <==

\begin{figure}[t]
    \centering
    \includegraphics[width=0.99\linewidth]{Styles/sections/figures/perceptual_error.pdf}
    \vspace{-3mm}
    \caption{
        \textbf{Example of Perceptual Error.}
    }
    \label{fig:perceptual_error}
\end{figure}


==> Styles/sections/src/temp.tex <==
Idefics2-8b & 28.9 & 28.1 \color{red}(-0.8) & 28.1 \color{red}(-0.8) \\
xGen-MM & 36.7 & 28.3 (-8.4) & 28.3 \color{red}(-8.4) \\
InternVL2-2B & 32.5 & 29.7 \color{red}(-2.8) & 28.6 \color{red}(-3.9) \\
EvoVLM JP v2 & 30.0 & 30.8 \color{blue}(+0.8) & 28.6 \color{red}(-1.4) \\
LLaVA-1.6-13B & 26.4 & 31.9 \color{blue}(+5.5) & 29.2 (+2.8) \\
Phi-3v & 35.0 & 31.7 \color{red}(-3.3) & 29.7 \color{red}(-5.3) \\
Idefics3-8b & 33.1 & 31.7 \color{red}(-1.4) & 29.7 \color{red}(-3.4) \\
LLaVA-OV-0.5B & 28.9 & 28.9 (±0.0) & 29.7 \color{blue}(+0.8) \\
Phi-3.5v & 39.2 & 33.6 \color{red}(-5.6) & 31.1 \color{red}(-8.1) \\
LLaVA-Calm2 & 29.4 & 28.3 \color{red}(-1.1) & 31.4 (+2.0) \\
Mantis 8B & 32.5 & 31.1 \color{red}(-1.4) & 31.4 \color{red}(-1.1) \\
CogVLM2-19B & 32.8 & 31.9 \color{red}(-0.9) & 34.4 \color{blue}(+1.6) \\
LLaVA-OV-7B & 45.0 & 38.3 \color{red}(-6.7) & 35.6 \color{red}(-9.4) \\
InternVL2-8B & 43.9 & 38.3 \color{red}(-5.6) & 37.2 \color{red}(-6.7) \\
LLaVA-1.6-34B & 43.6 & 40.8 \color{red}(-2.8) & 38.9 \color{red}(-4.7) \\
Gemini1.5Pro & 50.6 & 42.2 \color{red}(-8.4) & 42.2 \color{red}(-8.4) \\
GPT-4o & 48.1 & 55.3 \color{blue}(+7.2) & 53.1 \color{blue}(+5.0) \\

==> Styles/sections/src/textual_understanding.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.99\linewidth]{Styles/sections/figures/textual_understanding.pdf}
    \vspace{-3mm}
    \caption{
        \textbf{Example of Textual Error.}
    }
    \label{fig:textual_understanding}
\end{figure}


==> z.intro-keep.tex <==
%%%%% pattern 1 begin %%%%%
% Recent large multimodal models (LMMs) have demonstrated exceptional performance across various tasks, ranging from common-sense reasoning to those requiring expert-level, domain-specific knowledge.
% This highlights the critical role of benchmarks in guiding model development.
% For instance,~\citet{yue2024mmmu} has created MMMU benchmark to evaluate advanced reasoning capabilities across diverse subject areas.
% By providing a standardized measure of performance, MMMU serves as a compass for developers, directing their efforts towards continual improvement on its quantitative scores.
% Such advancements in LMMs, however, have mainly focused on its performance in English, less prioritizing the utility in other languages.
% In particular, the performance of LMMs in Japanese, despite its large number of speakers, does not gain enough attention.
% For instance, Japanese words represent only 0.1\% of the dataset used in training GPT-3, while > 92\% consists of English text~\cite{gpt3wordcount}.
% Given this situation, there is a growing concern that LMMs might be performing poorly in Japanese.
% \ke{Better if we have multimodal examples instead of GPT3.}

% \input{Styles/sections/src/fig_overview}

% Such concern fundamentally comes from the lack of a benchmark that reliably evaluates the performance and provides a direction for improvements in LMMs in Japanese.
% Most Japanese multimodal benchmarks are created by translating existing English benchmarks~\citep{javgvqa500,llavabenchja,llavabenchinthewild}.
% We believe this approach is insufficient as
% (i) the consisting questions are often unfamiliar to Japanese people and do not account for cultural difference, and
% (ii) despite the importance of multimodal reasoning, the images are left untranslated, ignoring the fact that there are English sentences. 
% For these reasons, there may be a gap between the scores provided by such benchmarks and the true performance perceived by Japanese users.
% There are some benchmarks that have been trying to address these issues~\citep{inoue2024heron,zheng2024judging,javlmbenchinthewild}.
% However, such benchmarks are often limited in size (only up to 102 questions~\citep{inoue2024heron}), raising concerns about whether reliable quantitative evaluation can be achieved.
% \ke{maybe add smth like ``Further, all of them focus on evaluating common-sense reasoning tasks, and none of them measures expert-level knowledge'' but i feel it's too much information.}
%%%%% pattern 1 end %%%%%




% In recent years, the development of Large Language Models (LLMs) has been remarkable, with significant improvements in performance. 
% These LLMs are trained on large datasets, enabling them to generate and understand natural language in a manner similar to humans. 
% Along with this progress, there has been growing interest in models that possess multimodal capabilities, integrating not only text but also other types of information such as images and audio—these are known as Large Multimodal Models (LMMs).
% LMMs hold promise for various applications, such as image caption generation, visual question answering, and multimodal translation, and are being actively developed around the world, both as open-source and closed-source projects \cite{GPT4o, chen2023internvl, li2024llava, liu2024llavanext}.

% \jb{代表としてmmbench + mmmuで十分？ ocr bench は有名ではなく、chartqaは2022なのでintroでは必要でなければ、遠慮したい}
% To evaluate these LMMs, a variety of benchmarks have been introduced. These include Optical Character Recognition (OCR) \citep{liu2024hiddenmysteryocrlarge}, the ability to understand graphs and charts~\citep{masry2022chartqa}, and specialized knowledge in fields such as science and medicine \citep{yue2024mmmu}. 
% These diverse evaluation metrics are important for the comprehensive assessment of LMMs, and they contribute to improvements and the developments of new application areas.

% % \jb{JPN benchをやる意味・理由も入れる}
% However, these benchmarks are created in English, and the performance evaluation of LMMs in other languages, including Japanese, has not progressed sufficiently.
% While some Japanese models \citep{akiba2024evomodelmerge, llavacalm2} have been released, there is a lack of appropriate evaluation when assessing their performance.

% Given the circumstance, we introduce \textbf{JMMMU} (\textit{Japanese MMMU}).
% The overview of JMMMU is shown in Figure \ref{fig:overview}.
% We translated the exsiting advanced LMM benhmark, MMMU (A Massive Multi-discipline Multimodal Understanding and Reasoning Benchmark), into Japanese and created new questions using images that reflect Japanese culture.


% Recent large multimodal models (LMMs) have demonstrated remarkable performance across various tasks, ranging from common sense reasoning to those requiring expert-level, domain-specific knowledge.

% This highlights the critical role of benchmarks in evaluating the diverse capabilities of LMMs.
% However, current benchmarks focus primarily on performance in English, with less emphasis on the utility in other languages.
% Notably, performance evaluations of LMMs in Japanese, despite its unique culture spreading around the world, remain underrepresented.
% Current Japanese multimodal benchmarks exhibit the following weaknesses:


% \vspace{-0.5em}
% \begin{itemize}[leftmargin=20pt]
%     % \setlength{\parskip}{0em} % 段落間
%     \setlength{\itemsep}{0.05em} % 項目間
%     \item \textbf{(W1)} Existing benchmarks~\citep{javgvqa,llavabenchja,llavabenchinthewild-JA,inoue2024heron,zheng2024judging,javlmbenchinthewild,ja-multivqa} focus on common sense knowledge, but none of them cover expert-level knowledge.
%     \item  \textbf{(W2)} Many of them do not account for cultural differences. They are often created by translating existing English benchmarks~\citep{javgvqa,llavabenchja,llavabenchinthewild-JA}, and thus the questions are unfamiliar to Japanese people.
%     \item  \textbf{(W3)} Recent benchmarks try to consider cultural differences~\citep{inoue2024heron,zheng2024judging,javlmbenchinthewild,ja-multivqa}, but they are all limited in size (only up to 102 questions~\citep{inoue2024heron}), raising concerns about whether reliable quantitative evaluation can be achieved.    
% \end{itemize}
% \vspace{-0.5em}

% \paragraph{This work: Creating a Massive, Expert-level, Truly-Japanese Multimodal Benchmark}
% Given the circumstance, we introduce \textbf{JMMMU} (\textit{Japanese MMMU}), a multimodal benchmark that can truly evaluate expert-level LMM performance in Japanese.
% An overview of our JMMMU can be found in~\Cref{fig:overview}.
% To address  \textbf{(W1)}, we created a benchmark based on MMMU~\citep{yue2024mmmu}, which is widely used to evaluate LMMs' expert-level reasoning with domain-specific knowledge.
% For  \textbf{(W2)}, we first carefully analyzed the existing MMMU benchmark for its cultural dependencies.
% Then, for questions in culture-agnostic subjects, we employed native Japanese speakers who are experts in each subject, and asked them to translate both the texts and images (e.g. the title of a graph) into Japanese.
% Further, we replaced culture-dependent subjects with new subjects that are conceptually similar, but better aligned with Japanese culture.
% For example, the original MMMU contains a subject called \textit{History}, which we divided into \textit{Japanese History} and \textit{World History}. For each subject, we sourced images from the web that had no licensing issues and created questions based on content typically found in Japanese textbooks.
% Finally, in response to \textbf{(W3)}, JMMMU consists of 720 translation-based (culture-agnostic) and 600 brand-new (culture-specific) questions, for a total of 1,320 questions, updating the size of the existing culture-aware Japanese benchmark by >10x.


% \paragraph{Implication of Our Benchmark Creation}
% % Our JMMMU benchmark reveals previously unnoticed deficiencies in Japanese language skills.
% Our JMMMU benchmark for the first time enables the community to reliably evaluate LMM's expert-level reasoning capabilities in Japanese.
% Our observations suggest that focusing solely on performance evaluation in English could risk a biased development competition that overlooks the utility in non-English languages.
% Conversely, a benchmark for a specific language can stimulate interest among model developers to improve its accuracy, as is currently observed with Chinese~\citep{zhang2024cmmmu,lu2024deepseek}.
% We hope that our benchmark will not only trigger the community's interest in Japanese language performance, but also serve as a catalyst for benchmark creation in other languages, leading to the development of LMMs that are more inclusive of non-English languages.

\paragraph{Contributions}
Our main contributions are:
\begin{itemize}
    \setlength{\parskip}{0cm} % 段落間
    \setlength{\itemsep}{0cm} % 項目間
    \item The largest dataset that reflects Japanese culture
    \item The Only dataset capable of measuring advanced capabilities in Japanese
    \item We reveal that there is room for improvement
\end{itemize}
